Do Different Tracking Tasks Require Different Appearance Models?

Tracking objects of interest in a video is one of the most popular and widely applicable problems in computer vision. However, with the years, a Cambrian explosion of use cases and benchmarks has fragmented the problem in a multitude of different experimental setups. As a consequence, the literature has fragmented too, and now novel approaches proposed by the community are usually specialised to fit only one specific setup. To understand to what extent this specialisation is necessary, in this work we present UniTrack, a solution to address five different tasks within the same framework. UniTrack consists of a single and task-agnostic appearance model, which can be learned in a supervised or self-supervised fashion, and multiple ``heads'' that address individual tasks and do not require training. We show how most tracking tasks can be solved within this framework, and that the same appearance model can be successfully used to obtain results that are competitive against specialised methods for most of the tasks considered. The framework also allows us to analyse appearance models obtained with the most recent self-supervised methods, thus extending their evaluation and comparison to a larger variety of important problems.

==> 2.tasks.tex <==
% \section{Taxonomy of Tracking Tasks}
% \label{sec:tasks}
% Existing tracking tasks can be categorized from multiple perspectives. In terms of target number, some tasks assume a single target while others deal with multiple objects. In terms of initialization, user-initialized tasks ask users to annotate targets only in \emph{one} certain frame, while auto-initialized tasks run detectors so that observations in \emph{every} frame can be attained. In terms of target object class, some tasks focus on tracking a given set of known classes, such as pedestrian and cars, while others are class-agnostic, able to track any object. In terms of observation format, tracking bounding boxes, segmentation masks, and pose skeletons are all of our interest. In this work, we involve six tasks: 

% \textbf{SOT} (Single Object Tracking)~\cite{otb}: User-initialized, single target, class-agnostic, box format.

% \textbf{VOS} (Video Object Segmentation)~\cite{davis}: User-initialized, single target, class-agnostic, mask format.

% \textbf{MOT} (Multiple Object Tracking)~\cite{mot16}: Auto-initialized, multiple target, class-specific, box format.

% \textbf{MOTS} (Multiple Object Tracking and Segmentation)~\cite{mots} and \textbf{VIS} (Video Instance Segmentation)~\cite{ytbvis}: Auto-initialized, multiple target, class-specific, mask format.

% \textbf{Pose Tracking~\cite{posetrack}}: Auto-initialized, multiple target, class-specific, pose format.

% Figure~\ref{fig:tasks} summarizes the involved tasks. Note that with above taxonomy we can easily derive other tracking tasks. One existing example is Tracking Any Object~\cite{tao}, a new setting that encourages algorithms to track open-class targets. Other examples include tasks undefined yet, such as tracking class-agnostic masks or poses. In this work, we dedicate to design a framework to solve the six listed tasks, meanwhile the framework is also potentially able to handle other tasks shown in Figure~\ref{fig:tasks}. 

% \begin{figure}
%   \includegraphics[width=\linewidth]{fig/teaser.pdf}
%   \caption{Existing tracking tasks differ with each other from muliple perspectives. The targets to be tracked are assumed to be a single object or multiple objects; targets can be specified by users or by automatic detectors; the classes of targets can be a close set (class-specific) or an open set (class-agnostic); the format of the targets can be bounding boxes, segmentation masks, or poses.} 
%   \label{fig:tasks}
% \end{figure}


